Smells and Refactorings for Software Environmental Sustainability: A Systematic Literature Review

Context: The environmental impact of ICT is constantly growing. Enhancing its environmental sustainability requires dealing with energy-hungry software systems, by possibly reducing their footprint. Objective: To better frame the problem and its persistent nature, software can be viewed as carrying structural inefficiencies regardless of how advanced its functionality may be. Identifying these inefficiencies as "green smells" provides a basis for refactoring code to mitigate its ecological impact. We aim at identifying well-known green smells impacting environmental sustainable software and map them to corresponding refactoring aimed at reducing the impact therein. Method: In this article, we conduct a systematic literature review on the articles that discuss green smells and their possible refactorings. We analyse and classify 66 primary studies published up to March 2026. Results: We identify 20 smells impacting environmental sustainability of software. Each smell is associated with one or more refactoring techniques known to mitigate their negative effects on the environmental sustainability of software. Conclusions: The literature witnesses the interest in resolving the green smells affecting software systems. The catalogued green smells and the corresponding refactorings can provide pragmatic value for practitioners in their daily development workflows, while also offering researchers a starting point to establish new research directions in sustainable software engineering.

==> tab/taxonomy_cardinality.tex <==

\scriptsize
\centering
% \begin{tabular}{ccl} %p{.78\textwidth}}

%     \hline 
%     \rowcolor{headergray}
%     \textbf{Total} & & \\ %\textbf{Total} \\
%     \rowcolor{headergray}
%     \textbf{Green smells} & \textbf{Green smell} & \textbf{Refactorings} \\
%     \hline
    
% 26 & Inefficient data structures & Use optimised data structures \\ 
% \rowcolor{rowgray}
% 24 & Multiple responsibility classes & Follow single responsibility principle \\

% 19 & Excessive looping    & Remove loop initialisation \\
%     &    & Separate exit condition \\
%     &    & Unroll nested loops \\
%     &    & Use optimised loop \\
    
% \rowcolor{rowgray}
% 18 & Durable resource usage & Lock resources only when necessary \\

% 17 & Heavy graphics    & View usage optimisation \\
%     &    & Avoid useless animation \\
%     &    & Dark colour usage \\
    
% \rowcolor{rowgray}
% 17 & Inefficient transmission    & Reduce payload \\
% \rowcolor{rowgray}
%     &    & Use dynamic retry delay \\

% 16 & Excessive encapsulation    & Reduce encapsulation \\

% \rowcolor{rowgray}
% 16 & Redundant code    & Remove obsolete code \\
    
% 16 & Excessive event rate    & Push over pull \\
%     &    & Reduce event rate \\
%     &    & Batch events \\
    
% \rowcolor{rowgray}
% 15 & Excessive indirection    & Reduce indirection \\
    
% 14 & Excessive delegation    & Reduce delegation \\

% \rowcolor{rowgray}
% 12 & Long function    & Decompose function \\

% 11 & Repeated computation    & Extract local variable \\
%     &    & Use caching \\
%     &    & Use pre-fetching \\
    
% \rowcolor{rowgray}
% 11 & Inefficient parallelism    & Avoid leaking threads \\
% \rowcolor{rowgray}
%     &    & Limit threads \\

% 11 & Wrong variable types    & Move global to local variables \\
%     &    & Move static to instance variables \\

% \rowcolor{rowgray}
% 10 & Inefficient algorithm    & Use optimised algorithm \\
    
% 8 & Inefficient third-party APIs    & Use energy-efficient APIs \\

% \rowcolor{rowgray}
% 7 & Single functioning    & Enable emergency mode \\
    
% 5 & Interpreted programming language    & Switch to compiled language \\

% \rowcolor{rowgray}
% 3 & Useless recursion      & Use iterative solution \\



\begin{tabular}{cclc} %p{.78\textwidth}}

    \hline 
    \rowcolor{headergray}
    \textbf{Total} & & &\textbf{Total} \\
    \rowcolor{headergray}
    \textbf{Green smells} & \textbf{Green smell} & \textbf{Refactoring} &\textbf{Refactorings} \\
    \hline
    
26 & Inefficient data structures & Use optimised data structures &23 \\ 
\rowcolor{rowgray}
24 & Multiple responsibility classes & Follow single responsibility principle &23\\

19 & Excessive looping    & Remove loop initialisation &6 \\
    &    & Separate exit condition &3 \\
    &    & Unroll nested loops &10\\
    &    & Use optimised loop &5\\
    
\rowcolor{rowgray}
18 & Durable resource usage & Lock resources only when necessary &9\\

17 & Heavy graphics    & View usage optimisation &6\\
    &    & Avoid useless animation &4\\
    &    & Dark colour usage &9\\
    
\rowcolor{rowgray}
17 & Inefficient transmission    & Reduce payload &13\\
\rowcolor{rowgray}
    &    & Use dynamic retry delay &2\\

16 & Excessive encapsulation    & Reduce encapsulation &12\\

\rowcolor{rowgray}
16 & Redundant code    & Remove obsolete code &10\\
    
16 & Excessive event rate    & Push over pull &4\\
    &    & Reduce event rate &8\\
    &    & Batch events &11\\
    
\rowcolor{rowgray}
15 & Excessive indirection    & Reduce indirection &14\\
    
14 & Excessive delegation    & Reduce delegation &10\\

\rowcolor{rowgray}
12 & Long function    & Decompose function &6\\

11 & Repeated computation    & Extract local variable &3\\
    &    & Use caching &7\\
    &    & Use pre-fetching &2\\
    
\rowcolor{rowgray}
% 11 & Inefficient parallelism    & Avoid leaking threads &7\\
\rowcolor{rowgray}
    &    & Limit threads &3\\

11 & Wrong variable types    & Move global to local variables &3\\
    &    & Move static to instance variables &5\\

\rowcolor{rowgray}
10 & Inefficient algorithm    & Use optimised algorithm &6\\
    
8 & Inefficient third-party APIs    & Use energy-efficient APIs &4\\

\rowcolor{rowgray}
7 & Single functioning    & Enable emergency mode &6\\
    
5 & Interpreted programming language    & Switch to compiled language &3\\

\rowcolor{rowgray}
3 & Useless recursion      & Use iterative solution &3\\



    \hline 
\end{tabular}








